A Goal-Driven Survey on Root Cause Analysis

Root Cause Analysis (RCA) is a crucial aspect of incident management in large-scale cloud services. While the term root cause analysis or RCA has been widely used, different studies formulate the task differently. This is because the term "RCA" implicitly covers tasks with distinct underlying goals. For instance, the goal of localizing a faulty service for rapid triage is fundamentally different from identifying a specific functional bug for a definitive fix. However, previous surveys have largely overlooked these goal-based distinctions, conventionally categorizing papers by input data types (e.g., metric-based vs. trace-based methods). This leads to the grouping of works with disparate objectives, thereby obscuring the true progress and gaps in the field. Meanwhile, the typical audience of an RCA survey is either laymen who want to know the goals and big picture of the task or RCA researchers who want to figure out past research under the same task formulation. Thus, an RCA survey that organizes the related papers according to their goals is in high demand. To this end, this paper presents a goal-driven framework that effectively categorizes and integrates 135 papers on RCA in the context of cloud incident management based on their diverse goals, spanning the period from 2014 to 2025. In addition to the goal-driven categorization, it discusses the ultimate goal of all RCA papers as an umbrella covering different RCA formulations. Moreover, the paper discusses open challenges and future directions in RCA.

==> chapters/legacy_inference.tex <==
\section{CHALLENGES OF INFERENCE}\label{sec:method}

In this section, we explore the various challenges related to the inference part of the methods. The discussion will cover key areas, including inference time, cost-effectiveness, robustness, scalability, incremental training, and the integration of human-in-the-loop approaches. By examining these dimensions, we aim to provide a comprehensive understanding of the factors that influence the efficiency and practicality of the algorithms under the scope of RCA.

\subsection{INFERENCE TIME}

Inference time is critical in evaluating root cause analysis (RCA) algorithms. Faster inference time enables quicker response to issues, minimizing downtime and improving system reliability. Lots of works address their quick inference time, we categorize this portion as techniques based on pruning~\cite{zhang2021halo,zhang2021onion,thalheim2017sieve,liu2021microhecl,ding2023tracediag,harsh2023murphy,wang2015methodology,he2022graph,li2021practical,zhang2024trace,yu2023cmdiagnostor,jiang2023look,li2022causal,ikram2022root,xie2024microservice}, parallel processing~\cite{zhang2024trace,gan2021sage,yu2023nezha,harsh2023murphy,li2022causal,lin2018microscope}.


\subsubsection{Reducing the search space}
Since the most input for RCA, i.e., telemetry data, often lacks failure-related information, irrelevant data can be quickly pruned, thereby accelerating the RCA process. Additionally, if the results generated by the algorithm do not meet certain thresholds or patterns, the process can be terminated early, further enhancing efficiency. Almost all methods~\cite{liu2021microhecl,zhang2024trace,ikram2022root,zhang2021onion,he2022graph,li2021practical,jiang2023look,harsh2023murphy} employ some form of pruning strategy to reduce the search space and improve efficiency. These strategies may involve similarity metrics (e.g., Pearson's correlation coefficient~\cite{abe2008analyzing} in MicroHECL~\cite{liu2021microhecl} and metric similarity pruning in CMDiagnostor~\cite{yu2023cmdiagnostor}), event features (e.g., event pruning and Chi-square pruning in TraceContrast~\cite{yu2023cmdiagnostor}), or topology (e.g., the DBSCAN algorithm~\cite{ester1996density} and influence topology filtering in GIED~\cite{he2022graph}). All these pruning strategies aim to eliminate irrelevant or low-relevance paths, nodes, or features to narrow down the problem and focus resources on deeper analysis.

Some methods organize and simplify the problem by exploiting the hierarchical nature of the data or structure.
TraceDiag~\cite{ding2023tracediag} is an adaptive and interpretable approach designed to enhance the efficiency of root cause analysis (RCA) in large-scale microservice systems. It leverages reinforcement learning (RL) to automatically learn a pruning policy that eliminates redundant components from service dependency graphs. This policy operates based on three main criteria: latency-based pruning, which removes components with low latency values; anomaly-based pruning, which filters out components with low anomaly indicators; and correlation-based pruning, which discards components with low correlation to end-to-end service latency. The RL-based pruning policy learns an optimal sequence of actions through a filtering tree, ensuring that the pruned graph retains only the components most relevant to RCA.
HALO~\cite{zhang2021halo} optimizes inference time by leveraging the hierarchical structure of telemetry data to reduce the search space intelligently. It begins by identifying and organizing attributes into an Attribute Hierarchy Graph (AHG), which guides an efficient attribute-level search phase. This phase strategically narrows down the focus to a subset of relevant attributes. Subsequently, a value-level search is conducted along the hierarchical paths defined by the AHG, employing a top-down approach coupled with an adaptive early-stopping mechanism to further minimize the number of attribute value combinations evaluated. Additionally, HALO~\cite{zhang2021halo} refines the search results through reverse truncation to enhance the compactness of the fault-indicating combinations, thereby significantly streamlining the fault localization process without the need for pruning techniques.
Onion~\cite{zhang2021onion} employs a ''downward-closure based pruning'' strategy during the clustering process, which stops the splitting process at an appropriate level, thus avoiding generating trivial log groups with low impact. This pruning strategy significantly improves efficiency by reducing unnecessary computations and focusing on critical information.
Sieve~\cite{thalheim2017sieve} reduces the search space by loading the application under various load conditions to obtain metrics and a call graph, reducing the dimensionality of metrics using clustering to identify representative metrics, and identifying dependencies between components using the call graph and Granger Causality tests. The call graph helps to reduce the number of component pairs that need to be checked for relationships. In contrast, clustering reduces the number of metrics to consider by selecting representative metrics from each cluster.
Squeeze~\cite{li2019generic} uses a “bottom-up then top-down” pruning strategy to accelerate anomaly root cause analysis while balancing speed and accuracy. In the bottom-up phase, the method filters normal attribute combinations and clusters potential abnormal ones based on their deviation scores, significantly reducing the search space. The top-down phase then localizes the root cause within each cluster using a heuristic approach guided by the generalized potential score (GPS), which enhances root cause identification by addressing cumulative forecast errors. This two-step approach efficiently narrows the search space and localizes root causes with improved precision and computational efficiency.

MicroHECL~\cite{liu2021microhecl} dynamically constructs a service call graph based on aggregated 30-minute window data. Starting with the initial anomalous service of availability issue, it utilizes a pruning strategy that eliminates irrelevant service calls by assessing the similarity of change trends in quality metrics between successive edges (service calls) in the propagation chain. Specifically, the Pearson correlation coefficient~\cite{abe2008analyzing} measures this similarity. If the coefficient is below a certain threshold, the edge is pruned, preventing the addition of potentially irrelevant anomalous nodes to the current anomaly propagation chain. 
Murphy~\cite{harsh2023murphy}, RCSF~\cite{wang2015methodology}, GIED~\cite{he2022graph} and TraceRCA~\cite{li2021practical} also use some kinds of thresholds to filter the unrelated intermediate results.
TraceContrast~\cite{zhang2024trace} first extracts the critical path, then transforms critical paths into event sets. Then, it identifies anomalous traces and affected paths. Using a parallel contrast sequential pattern mining algorithm, it uncovers candidate root causes. It mentions three types of pruning: Event pruning removes events unique to normal paths, Chi-square pruning eliminates patterns with a chi-square statistic value below a threshold when compared to their prefixes, and Minimum support pruning cuts off patterns with support lower than a specified threshold in the anomaly paths.
CMDiagnostor~\cite{yu2023cmdiagnostor} reduces the search space by using three key pruning strategies: AmSit-based Pruning (ASP), which removes irrelevant downstream paths; Metric Similarity-based Pruning (MSP), which eliminates paths where metric trends between successive calls are dissimilar; and Anomaly Detection-based Pruning (ADP), which prunes paths where metrics are normal. These strategies help focus the analysis on the most relevant parts of the graph, significantly narrowing down the potential root cause candidates.
TraceDiag~\cite{ding2023tracediag}uses three specific pruning methods to enhance root cause analysis by removing unnecessary nodes from trace data. The latency-based pruning method eliminates services with low latency metrics (such as average and maximum exclusive latencies) since they are less likely to be the root cause of an incident. The anomaly-based pruning method filters out components with low anomaly indicators, based on metrics like NormalizedCount and RankScore, as these services are unlikely to be involved in the incident. Lastly, the correlation-based pruning method removes nodes that show a low correlation between their latency and the overall end-to-end delay, as they are less likely to be relevant to the incident.
MicroCU~\cite{jiang2023look} implements pruning by enforcing a temporal order constraint on the path search within the temporal causal graph, ensuring that anomalies propagate in a strict time sequence. Applying this constraint, MicroCU~\cite{jiang2023look} eliminates paths that do not conform to the required temporal order, thereby reducing the number of generated paths and improving their relevance. Additionally, MicroCU~\cite{jiang2023look} validates paths based on causal peak timestamps, discarding those that fall outside the detected abnormal period. To further refine the search, it calculates path correlation strength while avoiding loops by restricting nodes to appear only once per path. The final ranking of potential root causes is determined by a weighted combination of path correlation strength and metric correlation strength, which together ensure that only the most relevant paths are considered, resulting in more accurate and efficient identification of root cause microservices.



\subsubsection{Parallel Processing}
Parallel processing is a common optimization methodology for speeding up the inference. TraceContrast~\cite{zhang2024trace} employs a parallelized contrast sequential pattern mining algorithm and Apache Spark’s distributed computing capabilities to identify and analyze patterns in large-scale trace data efficiently, enabling rapid identification of root causes in complex microservice systems. 
Sage~\cite{gan2021sage} trains its model in parallel.
Nezha~\cite{yu2023nezha} traverses the event graph and mines the pattern in parallel.
Murphy~\cite{harsh2023murphy} and CIRCA~\cite{li2022causal} support further optimization with parallelism support.
Microscope~\cite{lin2018microscope} uses a parallelized PC algorithm to construct causality graphs based on a single metric, and it leverages a conditioned graph traversing algorithm to locate the root cause. 



\subsection{COST EFFECTIVENESS AND ROBUSTNESS}
% 更少的输入量，但是可对比，甚至更好的效果
% Microrank 5.4.4 Impact of trace number. Our system is able to locate the root causes in the case of losing partial tracing data.
% robust Murphy, table2里描述了 robust
% robust Sage
% MicroCU
% Dycause. 6 自称即使输入指标减少了 $83.3\%$，DyCause 在结果准确性方面也优于几种最先进的方法。
Cost-effectiveness and robustness are crucial factors in assessing RCA algorithms since not all the systems can apply the monitoring infrastructure, and even those systems with the monitoring infrastructure, the collected data is will also lost~\cite{jiang2023look}. To this end, effective RCA solutions should provide accurate results with minimal resource expenditure and the ability to function with less input data while maintaining or even enhancing performance.

MicroCU~\cite{jiang2023look} only needs to use very sparse API logs to localize the root cause, based on the causal unimodalization, which effectively transforms causal curves into unimodal shapes, enhancing the interpretability and reliability of sparse data. Moreover, the dynamic causality discovery and the algorithm's robustness to different imputation methods contribute to its high accuracy, even under conditions of significant data sparsity.
SpanGraph~\cite{kong2024enhancing} demonstrates strong performance in few-shot learning scenarios, even with limited data. In tests using the SockShop~\cite{sockshop} and Trainticket~\cite{trainticket} datasets, SpanGraph achieved high F1 scores of 93\% and 88.95\% with just 1\% of the training data. The model’s performance improved across precision, recall, and F1-score as the data proportion increased. This highlights SpanGraph’s efficiency, reliability, and ability to generalize well with minimal data, making it a competitive solution for fault localization in microservices systems where data is scarce.

Microrank~\cite{yu2021microrank} uses trace data to construct the trace coverage tree. For normal and abnormal traces, it has normal and abnormal coverage trees. Based on the trace coverage tree, it constructs the real-time call graph for further root cause analysis. This method does not take care much of the single traces, on the other hand, it uses the statistical feature of the trace, thus, Microrank~\cite{yu2021microrank} can accept some data missing.
Similarly, Sage~\cite{gan2021sage} also constructs the Causal Bayesian Network by the traces, it does not require tracking individual requests to detect temporal patterns, making it robust to tracing frequency.
Murphy~\cite{harsh2023murphy} is even more robust in their evaluation since its use of a Markov Random Field (MRF) framework for reasoning in cyclic graphs, online model training to ensure up-to-date accuracy, counterfactual analysis for identifying root causes even without explicit causal data, and an efficient diagnosis process that prunes the search space to reduce complexity while maintaining precision.

Diagfusion~\cite{zhang2023robust} tackles two primary challenges: (1) representing diverse data formats and (2) addressing imbalanced failure types. To achieve this, DiagFusion~\cite{zhang2023robust} uses fastText~\cite{bojanowski2017enriching} for unified event representation across modalities, leveraging data augmentation to handle limited labeled data and imbalance in failure types. Additionally, it constructs a dependency graph from traces and deployment data to understand failure propagation paths and applies a graph neural network (GNN) to localize the root cause instance and classify the failure type.


\subsection{SCALABILITY}
% 能够承受更加大的输入量
% Groot，说之前的方法用的数据量都很少
Scalability refers to an algorithm’s ability to efficiently manage increasing volumes of data and complexity without a significant loss in performance. In the context of RCA, scalable solutions are crucial for handling the expanding volume and variety of hierarchical telemetry data generated by microservices.
To achieve high scalability, many approaches leverage the hierarchical nature of the data, dividing the original telemetry data into different levels of granularity and abstraction~\cite{wang2021groot,yao2024chain,ikram2022root}. Additionally, because most telemetry data does not indicate failure, algorithms can quickly prune data that lacks clear evidence of an issue, thereby avoiding unnecessary computations and enhancing scalability, as we mentioned in previous sections.

Groot~\cite{wang2021groot} and Chain-of-Event~\cite{yao2024chain} achieve scalability in RCA by constructing a global service dependency graph to map interactions across distributed systems. This graph allows Groot and Chain-of-Event to identify critical nodes that have a widespread impact on the system. The event graph aggregates low-level metrics, logs, and traces into higher-level features, reducing the data volume while preserving essential information, thus improving the scalability.
RCD~\cite{ikram2022root} employs a hierarchical learning approach by dividing the variables into smaller subsets and using the $\Psi$-PC algorithm to identify potential root causes within each subset. This method reduces the number of conditional independence (CI) tests needed, enhancing efficiency. After analyzing all subsets, RCD combines the results to identify candidate root causes. By focusing on localized learning around specific nodes (F-NODE), RCD further refines the potential root causes, improving both accuracy and runtime. This hierarchical strategy allows RCD to manage complex causal relationships more effectively.
HALO~\cite{zhang2021halo} first identifies the relationships among attributes to construct the Attribute Hierarchy Graph (AHG), then generates attribute search paths by performing random walk on AHG. The second phase contains a top-down search along the hierarchically arranged attribute paths to identify the best attribute value combinations. By using this technique, HALO can scale up to 1.2 million records.


\subsection{INCREMENTAL TRAINING}
% CORAL 增量训练
% sage 在线训练 section 4.4
% murphy 17
% spangraph 9

Change is common in microservice, there are service updates and service dependency changes every day. However, it is usually time-consuming and requires a large amount of data to train a robust model for new types of failure and dependency~\cite{wang2023incremental}.
Thus, incremental training (online training) is important for maintaining the relevance and accuracy of RCA algorithms over time. It involves updating the model continuously as new data becomes available, allowing the system to adapt to changing conditions and new failure patterns. To achieve this, there are commonly two ways: incremental training that adopts the new data to the model~\cite{gan2021sage,gan2023sleuth,wang2023incremental}, and online training that only uses fresh data~\cite{harsh2023murphy}.

\paragraph{Incremental training} CORAL~\cite{wang2023incremental} uses Long Short-Term Memory~\cite{hochreiter1997long} (LSTM) networks and Variational Graph Autoencoders~\cite{kipf2016variational} (VGAE) to capture both temporal and structural patterns in evolving data. Specifically, LSTM can remember long-term data features, allowing it to update its internal state incrementally with new data without the need for full retraining. When new telemetry data arrives, LSTM~\cite{hochreiter1997long} can continue to learn from this data based on its existing training results, thereby updating the model's prediction capabilities. This incremental learning approach avoids the need for full retraining with every data update, saving computational resources and enabling the model to adapt to new data distributions quickly. For VGAE~\cite{kipf2016variational}, incremental learning is realized through the updatability of the graph structure. The service dependency graph in a microservice system is often dynamic, with services being added, removed, or dependencies changing. During incremental learning, VGAE~\cite{kipf2016variational} updates the graph structure and its latent representations (embeddings) locally, rather than rebuilding the entire graph model.
For the same target, Sage~\cite{gan2021sage} utilizes Graph Variational Autoencoders (GVAE) and Causal Bayesian Networks (CBN) to implement incremental learning in response to changes in a microservice architecture. The GVAE allows for dynamic reshaping and incremental updates by adjusting the network structure and parameters without retraining the entire model. Meanwhile, the CBN captures and updates causal relationships between microservices, guiding selective retraining based on changes in the RPC graph or performance metrics. Together, these components enable Sage~\cite{gan2021sage} to efficiently adapt to microservice changes, reducing retraining time and maintaining model accuracy by updating only the relevant parts of the model and preserving causal integrity.
Sleuth~\cite{gan2023sleuth} improves upon Sage~\cite{gan2021sage} by using Graph Neural Networks (GNNs) to enable few-shot and zero-shot learning, allowing it to quickly adapt to new microservice applications with minimal data. Unlike Sage~\cite{gan2021sage}, which relies on GVAE and CBN for incremental updates, Sleuth’s GNN architecture captures generalizable patterns across different microservices, reducing the need for extensive retraining. This makes Sleuth more scalable and efficient, especially in dynamic environments where rapid deployment and high accuracy are essential.

Different from the previous papers, Murphy~\cite{harsh2023murphy} is inherently an online training method. Every time Murphy is called, it utilizes data from the week before the incident. This ensures that the models are continuously updated with the latest application topology and software versions, avoiding the use of outdated data. Including the most recent incident data is crucial, as it allows the model to capture new metrics patterns that may not have occurred previously, enhancing the accuracy of fault diagnosis. Additionally, another advantage of online training is that data points from the incident itself are included in the training. For instance, if the incident has been ongoing for 15 minutes when the operator invokes Murphy, those 15 minutes of real-time data will be incorporated into the training, further improving the model’s diagnostic capabilities.

\subsection{HUMAN IN THE LOOP}

% HRLHF RL+人工构建更加准确的因果图
% Déjàvu
% groot 15

Integrating human expertise into the Root Cause Analysis (RCA) process can significantly enhance the findings' accuracy and contextual relevance. Human-in-the-loop approaches, which combine algorithmic analysis with human insights, create a more robust and adaptable system. However, incorporating human input can sometimes require substantial effort. Thus, better utilization of human domain knowledge is an important topic.
Humans can incorporate into multiple processes, including preparing high-quality inputs~\cite{li2022causal, li2022actionable, wang2021groot,ma2020diagnosing,wang2023root} and the evaluation process~\cite{li2022actionable,yu2023nezha,chen2024automatic,zhang2024automated,zhang2024lm,ahmed2023recommending}.

\paragraph{Inputs} Groot~\cite{wang2021groot} allows Site Reliability Engineers (SREs) to add new event types, construct event graphs, and maintain rules for filtering and building these graphs. This capability enables human experts to inject their knowledge directly into the RCA system. However, it also introduces the overhead of manual configuration. To mitigate this, Chain-of-Event~\cite{yao2024chain} leverages historical incidents to automatically learn a Naive Event Graph while still allowing experts to refine parameters, thereby ensuring more effective utilization of human knowledge. 
Similar to Groot~\cite{wang2021groot}, Déjàvu~\cite{li2022actionable}, 
LogKG~\cite{sui2023logkg},
CIRCA~\cite{li2022causal} and iSQUAD~\cite{ma2020diagnosing} require engineers to label the correctness of the result during the process or provide some predefined pattern to help the model to distinguish the root cause better. To stimulate the real environment, MEPFL~\cite{zhou2019latent} needs student volunteers to play the role of users and manually execute the scenarios that may involve the target microservice. MicroCause~\cite{meng2020localizing} needs professional operators to manually collect the online failure ticket and find out the actual root cause.
HRLHF~\cite{wang2023root} draws inspiration from the outstanding results of Reinforcement Learning with Human Feedback (RLHF) in aligning large language models (LLMs) with human intent during training, effectively utilizing human feedback to reduce the uncertainty in dependency graph discovery. By integrating human feedback into reinforcement learning, HRLHF aims to construct dependency graphs with high accuracy while minimizing the need for human intervention.
TraceDiag~\cite{ding2023tracediag} leverages reinforcement learning (RL) to acquire an automated, interpretable, and adaptable pruning policy that effectively removes redundant components, enhancing the efficiency and accuracy of the RCA process. The policy is based on graph pruning rules derived from experienced engineers and comprehensive trace analysis, ensuring domain knowledge and industry best practices are incorporated. The pruned service graph is then utilized for RCA using causal methods.

\paragraph{Evaluation} There are no ground truth root causes in the actual industry service. Thus, in most cases, humans play an evaluation role to validate the performance of the RCA methods. Nezha~\cite{yu2023nezha} generates a suspicion list for SRE to check, which enables SRE to manually filter the miss-alarm.  
SynthoDiag~\cite{zhang2024fault}, it is deployed to online service and needs SREs to manually check the performance of the RCA methods.
RCACopilot~\cite{chen2024automatic}, FSE Companion'24~\cite{zhang2024automated}, LM-PACE~\cite{zhang2024lm} and ICSE'23 ~\cite{ahmed2023recommending} are four papers utilizing Large Language Model in root cause analysis, all of them needs human experts to evaluate the result. The human evaluation also needs to be simple, otherwise it also will cost lots of human effort. GMTA~\cite{guo2020graph}, Eadro~\cite{lee2023eadro}, and Groot~\cite{wang2021groot} all provided a user-friendly interface to interact with SREs.

\paragraph{Others} 
Some works only target to reduce the effort of looking up the redundant and large volume telemetry data, thus speeding up the operator to make decisions of which component is the root cause.
For example, the aim of GMTA~\cite{guo2020graph} is to visualize the trace graph and do further analysis of visualizing service dependencies, making architectural decisions, analyzing the changes in service behaviors, detecting performance issues, and locating root causes. It does not directly output a list of root cause candidates. More human effort is needed to inspect the anomaly manually.


==> chapters/legacy_input.tex <==
\section{CHALLENGES OF INPUT}\label{sec:input}
\label{sec:constraint}
In this section, we discuss the challenges associated with input data for RCA. 
As illustrated in Sec.~\ref{sec:constraint}, achieving effective RCA requires sufficient observational data, which increases computational/storage costs.
Starting from the constraint, we divide the challenges of input into two main parts: 
(1) The first part deals with the case that there are always blind spots that we cannot observe due to various reasons (Section~\ref{sec:blindspot}).
% For example, many metric/service level heterogeneous root cause candidates exist with limited observability in real-world microservices systems \cite{xie2024microservice}.
% To address this, some methods use models with reasoning techniques to reduce the need for missing data, effectively filling in the blind spots. 
% This method is particularly useful when storage and collection resources are limited, but it may struggle with inference accuracy. 
(2) The second part focuses on how to model the complexity of the input since the input data of RCA can be heterogeneous, multi-source, and multi-dimensional (Section~\ref{sec:complexity}).
They all describe the same runtime system, but each focuses on different components.
Unlike the first part, this part discusses the challenges encountered when most observational data are collected without considering the computational/storage constraints.
% Additionally, we also discuss the current practice of RCA. For example, the role of Anomaly Detection (Section~\ref{sec:anomalydetection})
Additionally, since Anomaly Detection (AD) is a precursor to the RCA process, the quality of AD results is crucial for ensuring accurate RCA. 
In Sec.~\ref{sec:anomalydetection}, we presented previous works addressing AD inaccuracies.


\begin{table}
\centering
\caption{Challenges of Input}
\resizebox{\textwidth}{!}{  % 调整表格大小，使其适应页面宽度
\begin{tblr}{
  cell{1}{2} = {c=3}{},
  cell{2}{1} = {r=5}{},
  cell{2}{2} = {r=4}{},
  cell{2}{3} = {r=3}{},
  cell{5}{3} = {c=2}{},
  cell{6}{2} = {c=3}{},
  cell{7}{1} = {r=5}{},
  cell{7}{2} = {c=3}{},
  cell{8}{2} = {c=3}{},
  cell{9}{2} = {c=3}{},
  cell{10}{2} = {c=3}{},
  cell{11}{2} = {c=3}{},
  cell{12}{2} = {c=3}{},
  hline{1,2,6,12,13} = {-}{0.08em},  % 添加水平分割线
  hline{7} = {1-5}{0.08em},  % 中间水平分割线
  vline{2,5} = {-}{0.08em},  % 竖直分割线
  hline{7} = {1-5}{0.08em},  % 中间水平分割线
  vline{3} = {1-5}{0.08em},  % 竖直分割线
  vline{4} = {1-4}{0.08em},
  hline{5} = {2-4}{0.08em}
}
\textbf{Category}        &        \textbf{SubCategory}             &                  &               & \textbf{Paper}                                                                                                                                                                                                                                                                                                                                                                 \\
\textbf{Blind Spots}     & Causal Discovery                     & Constraint-based & PC-based      & \cite{lin2018microscope,wang2018cloudranger,chen2014causeinfer,meng2020localizing,wang2023root,ma2021servicerank,zhang2021cloudrca} \\
                &                                      &                  & Granger-based & \cite{pan2021faster,thalheim2017sieve,jiang2023look,chen2023frl,mariani2018localizing,zhang2024illuminating,hu2022ts} \\
                &                                      &                  & Other         & \cite{yao2024chain,lu2022generic,nie2016mining}                                                                                                                                                                                                                                                                                                                       \\
                &                                      & Learning-based   &               & \cite{harsh2023murphy,zheng2024mulan,gan2021sage,gan2023sleuth,jeyakumar2019explainit,wang2023interdependent,wang2023incremental}                                                                                                                                                                                                                                     \\
                & Causal Inference                     &                  &               & \cite{xie2024microservice}                                                                                                                                                                                                                                                                                                                                            \\ 
\textbf{Data Complexity} & Intricate Service Dependencies       &                  &               & \cite{yu2024changerca,wang2023interdependent,liu2020unsupervised, wu2020performance, lin2018microscope, somashekar2024gamma, ma2020automap,wu2020microrca,ma2021servicerank,kim2013root,lin2018facgraph,chen2023frl,yang2022robust}                                                                                                                                   \\
                & Multidimensional Data Complexity     &                  &               & \cite{zhang2024trace,yan2022cmmd,meng2020localizing,zheng2024mulan, ma2020automap,nguyen2013fchain,ma2019ms,liu2019fluxrank,zhang2023robust, yang2022robust, lin2018microscope, jiang2023look}                                                                                                                                                                         \\
                & Data Path Ambiguity                  &                  &               & \cite{yu2023cmdiagnostor,he2022graph,ding2023tracediag,jia2017approach}                                                                                                                                                                                                                                                                                               \\
                & Scarcity of Incident-Related Data    &                  &               & \cite{yu2021microrank,liu2022microcbr,zhang2023robust}                                                                                                                                                                                                                                                                                                                 \\
                & Difficulty in Obtaining Labeled Data &                  &               & \cite{shan2019diagnosis, pham2024baro, gan2021sage, li2022causal, xie2024microservice, zhang2021onion, yu2023nezha, gan2023sleuth}                                                                                                                                                                                                                      \\          
\end{tblr} 
}
\label{tab:techniques_summary}
\end{table}


\subsection{REDUCING BLIND SPOTS THROUGH INFERRING UNOBSERVED DATA} \label{sec:blindspot}

As shown in Table. \ref{tab:techniques_summary}, the limitations in the input data arise from two main factors. The first is the absence of topology information. Since failures propagate across services, tracing error propagation typically requires constructing a graph to infer dependencies. However, in some cases, the service topology (or the associated tracing data) is either unavailable or difficult to obtain. For instance, there may be a lack of appropriate monitoring tools, leaving only service metrics as available data. In such cases, inferring or constructing possible relationships based on the observed data (e.g., metrics) is necessary.
The second factor is the incomplete availability of telemetry data. For example, direct telemetry data for a specific component under monitoring may be missing, leaving only indirect observations, such as data from third-party services. In such scenarios, causal inference techniques are employed to infer the unobserved data.

\subsubsection{Construct Graph by Causal Discovery}
%%%%%为什么使用causal discovery 
% 微服务之间的依赖关系会导致性能问题沿着服务链传播，从而引起不确定的服务质量（QoS）下降。因此，识别这些依赖关系对于准确诊断性能问题的根本原因至关重要。

% 通过学习因果结构可以捕捉微服务拓扑中的依赖关系，进而推断每个微服务的性能波动是如何影响整个系统的。这样就可以有效应对复杂的性能调试挑战 \cite{sage}
In microservice architectures, dependencies between services can cause issues to propagate along service chains, leading to unpredictable degradation in Quality of Service (QoS). 
Therefore, identifying these dependencies is crucial for accurately diagnosing the root causes of microservice issues.
By learning the causal structures within microservice topologies, we can capture these dependencies and infer how disruptions in one microservice affect the entire system. \cite{gan2021sage}.
%%%%
% 可以分为基于约束和基于学习两类
Causal discovery methods can be divided into constraint-based and learning-based approaches. 
Constraint-based methods excel in smaller, well-defined microservice systems with clean data, offering high interpretability through statistical tests \cite{yao2024chain}.
In contrast, learning-based methods are better suited for large-scale, dynamic environments with complex, nonlinear dependencies, handling noisy or incomplete data more effectively and scaling to higher dimensions \cite{gan2023sleuth}.

\textbf{Statistical-based graph construction.}
Statistical-based graph construction refers to a set of techniques that use statistical methods to infer causal relationships between different components in a system. 
By analyzing data—most commonly time series metrics—these methods construct causal graphs that represent how variables influence one another.
These graphs help in diagnosing system failures by identifying potential root causes through causal dependencies.

%%%PC-based
%%These methods use PC or itsvariant to construct a causal graph from time series metrics data and use a scoring method to locate the root cause.
% Microscope; causal
% CloudRanger; causal
% CauseInfer; causal
% MicroCause; causal
% HRLHF; causal
% ServiceRank; causal
% CloudRCA;causal
\textit{PC-based methods.}
The PC (Peter-Clark)~\cite{spirtes2001causation} algorithm is a widely used constraint-based method that constructs causal graphs step-by-step through a series of conditional independence tests. 
It systematically removes edges between conditionally independent variables, leaving only the most likely causal connections. 
This method is particularly effective in high-dimensional data environments, such as large-scale microservice systems with complex operational metrics. 
Examples of PC-based methods include Microscope~\cite{lin2018microscope}, CloudRanger~\cite{wang2018cloudranger}, CauseInfer~\cite{chen2014causeinfer}, MicroCause~\cite{meng2020localizing}, HRLHF~\cite{wang2023root}, ServiceRank~\cite{ma2021servicerank}, and CloudRCA~\cite{zhang2021cloudrca}.
MicroCause~\cite{meng2020localizing} improves the traditional PC algorithm by addressing its limitations in handling time series data. 
The PCTS (Path Condition Time Series) algorithm enhances the PC algorithm by capturing the propagation delays between different monitoring metrics, which the original PC algorithm overlooks by assuming data is independent and identically distributed (iid). 
Additionally, PCTS simplifies the causal graph by representing each node as a monitoring metric, rather than individual time points, making the graph more manageable for root cause analysis. 

%%%Granger-based
% DyCause；causal
% Sieve; causal
% MicroCU; causal
% FRL-MFPG; causal
% LOUD; causal
% GrayScope; causal
% TS-InvarNet; causal
\textit{Granger-based methods.}
Granger causality is primarily used for time series data. 
It tests whether the past behavior of one microservice helps predict another, allowing the identification of time-dependent causal relationships.  
For example, DyCause~\cite{pan2021faster} uses Granger causality testing to analyze dependencies between microservices. 
It collects performance metrics like request latency, and when an anomaly is detected, it applies a sliding window to the time series data.
In each window, Granger causality testing checks if the historical data of one service can improve the prediction of another service’s future state. 
If so, it indicates a causal relationship between the services, helping to build a dynamic causality map over time. This method is beneficial when the system involves microservices whose interactions evolve over time.
Granger-based techniques include DyCause~\cite{pan2021faster}, Sieve~\cite{thalheim2017sieve}, MicroCU~\cite{jiang2023look}, FRL-MFPG~\cite{chen2023frl}, LOUD~\cite{mariani2018localizing}, GrayScope~\cite{zhang2024illuminating}, and TS-InvarNet~\cite{hu2022ts}.


\textit{Other methods.}
%%% NEG
% chain of event; causal
Chain-of-Event \cite{yao2024chain} uses the Chain-of-Event (CoE) model for causal discovery, automatically learning causal relationships between events from historical data. 
It first generates a naive event-causal graph (NEG) that connects all potentially related events. 
Then, the CoE model automatically learns the causal link weights and event importance scores, avoiding manual configuration and improving accuracy. 
By tracing event chains, the model calculates root cause scores for each event, identifying the most likely root cause. 
%%%G-GES (Group-based Greedy Equivalent Search)
% CauseRank; causal
CauseRank~\cite{lu2022generic} introduces G-GES (Group-based Greedy Equivalent Search), a causal discovery algorithm that is part of the CauseRank method, designed to tackle performance diagnosis challenges in Online Transaction Processing (OLTP) systems. 
G-GES groups related metrics and uses these groups as nodes to build a simpler causal graph.
By incorporating domain knowledge, such as DBAs’ expertise and known system dependencies, G-GES improves the accuracy of identifying failure paths. 
It addresses three key challenges: 1) managing large numbers of abnormal metrics, 2) modeling complex failure propagation, and 3) ensuring efficient and accurate fault localization.
%%%FP-GROWTH
% IPCCC’16; causal
In IPCCC’16 \cite{nie2016mining}, the initial causal graph is built using the FP-Growth algorithm.
The system mines historical monitoring data to find associations between symptom events, identifying potential causal rules.
These frequent co-occurrences form the initial causal graph, which is then used for root cause analysis. 
At this stage, the graph is purely data-driven, relying on patterns in historical data without requiring prior knowledge.

\textbf{Learning-based graph construction.}
%%%Markov Random Field, MRF
% Murphy; causal
Traditional methods like the PC algorithm fail to handle cyclic dependencies and unclear relationships common in enterprise networks and microservices.
Murphy~\cite{harsh2023murphy} employed Markov Random Field~\cite{li2009markov} (MRF), a probabilistic model that allows cycles and bidirectional dependencies in the graph.
By learning joint distributions from historical data and applying Gibbs sampling for inference, the MRF model effectively captures complex interactions, improving the accuracy of root cause analysis in these environments.
%%% VAR
%%基于分数驱动方法，并使用了Vector Autoregression (VAR) 模型进行因果关系的建模。VAR模型通过历史时间序列数据捕捉系统实体之间的因果关系，能够有效地处理多模态数据之间的复杂相互作用。选择VAR模型的原因在于其能够在时间序列中捕捉变量之间的动态依赖关系，并通过结合图神经网络来处理非线性关系。这种方法特别适合处理微服务系统中的多模态数据，因为它可以综合考虑系统日志、性能指标等多种数据来源，提供更准确的因果图结构，帮助识别系统中的根因故障
% MULAN; causal
MULAN~\cite{zheng2024mulan} uses the Vector Autoregression (VAR) model to capture dynamic causal relationships between system entities from historical time-series data.
The VAR model is well-suited for handling multi-modal data, like system logs and performance metrics, as it can model the interactions between different data sources. 
It also predicts future values based on past observations. 
%%%Causal Bayesian Networks (CBN)
% ExplainIt; causal
% Sage; causal
% Sleuth; causal
Causal Bayesian Networks (CBN) are graphical models that represent causal relationships using Directed Acyclic Graphs (DAGs), where nodes are variables and edges show causal dependencies.
CBN constructs causal graphs by analyzing data or system structures, leveraging conditional independence to simplify complex relationships.
CBN-based techniques include Sage~\cite{gan2021sage}, Sleuth~\cite{gan2023sleuth} and ExplainIt~\cite{jeyakumar2019explainit}.
%%%TCD
% REASON; causal ；+ICD
The Topological Causal Discovery (TCD) in REASON~\cite{wang2023interdependent} uses hierarchical graph neural networks to construct causal graphs between system entities.
It captures both within-level and cross-level causal relationships, creating a comprehensive map of how system components are interconnected causally.
%%%Incremental Disentangled Causal Graph Learning (IDCGL)
% CORAL; causal
CORAL~\cite{wang2023incremental} uses an Incremental Disentangled Causal Graph Learning method for causal discovery. 
It separates causal relations into “state-invariant” and “state-dependent” types. 
As new data comes in, the causal graph is updated incrementally, adjusting only the state-dependent relations while keeping the state-invariant ones unchanged. 
This approach efficiently handles real-time data, enabling quick updates to the causal graph for root cause identification.


\subsubsection{Infer Beyond Observation by Causal Inference}

Previous causal inference methods rely on good observability~\cite{li2022causal,xie2024microservice,gan2021sage,harsh2023murphy,gan2023sleuth,ikram2022root}. 
For example, CIRCA~\cite{li2022causal} uses Regression-based Hypothesis Testing (RHT) to detect vanishing causal relationships between metrics and identify faults.
However, its effectiveness is limited because it requires all relevant variables to be observable, which is often not feasible in complex microservice environments where data can be missing or incomplete. 
% LatentScope addresses the limitations of previous causal inference methods, such as CIRCA, which require full observability of variables. In complex microservice environments, this is often not feasible due to missing or incomplete data. To overcome this, LatentScope models root cause candidates (RCCs) as latent variables, inferring their state through related observable metrics. It constructs a dual-space graph that separates latent RCC variables from observable metrics, enabling it to manage heterogeneous and unobservable RCCs efficiently. LatentScope introduces the Regression-based Latent-space Intervention Recognition (RLIR) algorithm, which performs fast inference and identifies root causes by analyzing causal relationships between latent and observable variables.
% To address this limitation, LatentScope~\cite{xie2024microservice} models RCCs as latent variables and uses related observable metrics to infer their status. 
% It introduces a dual-space graph to separate observable and latent variables, and employs the RLIR algorithm for fast and accurate root cause analysis, even with limited observability.

LatentScope~\cite{xie2024microservice} overcomes the limitations of previous causal inference methods. 
In complex microservice environments, full visibility is often unfeasible due to missing or incomplete data.
To address this, LatentScope models root cause candidates (RCCs) as latent variables and infers their states through related observable metrics. 
It constructs a dual-space graph that separates latent RCCs from observable metrics, allowing it to effectively manage heterogeneous and unobservable RCCs. 
LatentScope also introduces the Regression-based Latent-space Intervention Recognition (RLIR) algorithm, which quickly infers and identifies root causes by analyzing the causal relationships between latent and observable variables.
While Sage~\cite{gan2021sage} also mentions latent variables, it primarily uses them to capture system randomness, such as server performance fluctuations or network delays, and still heavily depends on observable data for causal inference. 
This reliance means that Sage’s effectiveness diminishes significantly when data is incomplete or missing.
In Sage, latent variables are mainly used to explain performance fluctuations rather than to solve the problem of unobserved root causes.
In contrast, LatentScope places latent variables at the core of its causal inference process.
By modeling unobservable RCCs as latent variables and inferring them with observable data, LatentScope directly addresses the challenges of missing or unobservable data. 
Its dual-space graph and RLIR algorithm further enhance its ability to connect and separate latent RCCs from observable metrics, providing accurate root cause analysis even with limited observability.



% latentscope; causal


% Causal inference-based approaches are particularly powerful when dealing with latent variables and missing information.
% To reduce the need for unobserved data, reasoning techniques such as the generation of counterfactuals are employed~\cite{li2022causal,xie2024microservice,gan2021sage,harsh2023murphy,gan2023sleuth,ikram2022root}.
% Traditional methods in cloud performance debugging often rely on supervised learning and intervention-based approaches, which necessitate extensive real-time data labeling and intervention.
% Such real-time operations are impractical for large-scale production environments. 
% Instead, Sage~\cite{gan2021sage}, a pioneer work on counterfactual analysis, utilizes an unsupervised learning approach based on generating counterfactuals.
% This approach leverages a Conditional Variational Autoencoder (CVAE)~\cite{sohn2015learning} to learn the distribution of latent variables from historical data and generate counterfactual scenarios. 
% These scenarios simulate the system’s behavior under different conditions, helping to identify potential issues that may not have been observed previously but could impact current performance.
% By using this method, Sage can accurately identify the root causes of Quality of Service (QoS) violations without the need for real-time intervention and labeled data.

% In contrast to Sage, Sleuth~\cite{gan2023sleuth} integrates GNNs into its counterfactual reasoning framework. 
% This eliminates the dependence on specific graph structures. 
% This innovation enhances Sleuth’s flexibility in dealing with different and evolving microservice architectures. 
% Furthermore, Sleuth’s use of few-shot learning broadens its applicability across diverse applications without the need for extensive retraining.

% In real-world enterprise environments, cyclic dependencies are common, but Sage relies on directed acyclic graphs (DAGs) to model causal relationships between microservices. 
% This makes Sage ineffective in handling systems with cyclic dependencies, limiting its accuracy in root cause analysis. 
% Murphy~\cite{harsh2023murphy}, on the other hand, uses a Markov Random Field (MRF)~\cite{besag1974spatial} model, which can naturally handle cycles and bidirectional dependencies, making it more suited to complex architectures.

% The effectiveness of Sage is also limited by its underlying assumption that no intervention has occurred in the system, which may not hold true in many real-world scenarios. 
% To address this, CIRCA~\cite{li2022causal} introduces the concept of Intervention Recognition (IR). 
% Unlike Sage, which relies on counterfactual scenarios, CIRCA views system faults as interventions within a causal framework and identifies these interventions through changes in the conditional probability distributions within a Causal Bayesian Network (CBN)~\cite{pearl1995causal}.
% By constructing a CBN based on the system’s architecture and applying regression-based hypothesis testing, CIRCA can effectively recognize the root causes of system anomalies even when interventions occur. 
% This method not only improves the accuracy of root cause analysis but also enhances the explainability of the results, making it a more robust solution for complex online service systems. 
% % In contrast to Sage, CIRCA’s ability to detect and adjust for interventions in real-time provides a significant advantage in maintaining Quality of Service (QoS) and quickly mitigating faults.

% RCD~\cite{ikram2022root} addresses reasoning about unobserved data by modeling failures as interventions. 
% Unlike CIRCA, which relies on domain knowledge, static rules, and call graphs, it avoids these dependencies.
% RCD uses localized and hierarchical learning to solve this. 
% It treats failures as interventions and uses changes in data distributions to identify root causes, without external graph information. 
% By focusing on relevant parts of the causal structure, RCD reduces complexity and avoids the need for global causal graphs, making it more scalable and flexible.

% LatentScope~\cite{xie2024microservice} offers a key improvement over CIRCA in root cause analysis for microservices. 
% CIRCA relies on CBNs to model and identify the root cause based on observable variables. 
% However, CIRCA’s effectiveness is limited because it requires all relevant variables to be observable, which is often not feasible in complex microservice environments where data can be missing or incomplete. 
% To address this limitation, LatentScope~\cite{xie2024microservice} introduces an innovative approach by modeling root cause candidates (RCCs) as latent variables. 
% This allows for root cause analysis even when direct observations are unavailable, which ensures more accurate identification of issues in complex and heterogeneous systems.



\subsection{ADDRESSING DATA COMPLEXITY CHALLENGES} \label{sec:complexity}
As illustrated in Table. \ref{tab:techniques_summary}, several challenges persist due to the complexity inherent in the data, even when sufficient observational data is available.

To begin with, tracing causal fault propagation is particularly difficult because of the intricate cross-layer service dependencies involved~\cite{yu2024changerca}. 
Moreover, the multi-dimensional nature of the data, including the complex relationships between system metrics and logs, further complicates the analysis process~\cite{yan2022cmmd, zhang2024trace}. In addition, complex datasets often result in the construction of graphs with ambiguous data paths, where this ambiguity in call graphs can lead to inaccurate root cause identification~\cite{yu2023cmdiagnostor}. 
Furthermore, incident-related data tends to be much scarcer than normal operational data, especially within the same timeframe, making it difficult to gather sufficient information for effective analysis. 
Finally, even if adequate incident-related data is collected, ground truth labels for root cause analysis are typically unavailable in industry settings. Such information is usually only obtainable post-incident after the SRE team has detected and resolved the issue, and telemetry data has been stored for subsequent post-mortem analysis.

% ChangeRCA~\cite{yu2024changerca}
% REASON~\cite{wang2023interdependent}

\subsubsection{Intricate Service Dependencies}

In microservice architectures, intricate and dynamic dependencies between services create significant challenges for anomaly detection, fault propagation analysis, and root cause identification. 
These dependencies are complex and multifaceted, shaped by several factors such as frequent updates, asynchronous interactions, and the lack of centralized control. Additionally, the complexity is further exacerbated by diverse and evolving business logic dependencies, heterogeneous communication protocols, and the high degree of service autonomy. This makes it difficult to maintain accurate, up-to-date models of the system, further complicating efforts to ensure system reliability and timely issue resolution.
To address these challenges, researchers have proposed various methods, which can be grouped into two main categories based on how they tackle issues related to intricate service dependencies.

\textit{Maintaining an accurate model of service dependencies.}
Static dependency graphs quickly become outdated, hindering effective monitoring and diagnosis. 
To overcome this, several approaches focus on dynamically constructing or updating service dependency models that reflect the current state of the system in real-time.
ServiceRank~\cite{ma2021servicerank} constructs an Impact Graph based on real-time monitoring data, dynamically determining causal relationships between services without relying on a static system topology. 
This method adapts to the evolving nature of microservices, capturing current service interactions and enhancing the accuracy and efficiency of root cause identification.
FacGraph~\cite{lin2018facgraph} captures the system’s changing topology during both normal and abnormal states by using correlation graph construction. 
Employing a PC-algorithm-based correlation graph, FacGraph dynamically maps out service dependencies as they evolve and utilizes Frequent Subgraph Mining to identify recurring anomaly patterns. 
This approach allows for pinpointing root causes without constant centralized monitoring, reducing overhead and improving efficiency.
Microscope~\cite{lin2018microscope} automatically discovers service dependencies by analyzing network-related system calls, such as \texttt{socket()} and \texttt{connect()}. 
This method accurately captures real-time dependencies without modifying source code or relying on potentially error-prone statistical inference. 
By directly monitoring system interactions, Microscope~\cite{lin2018microscope} ensures precise dependency mapping, enhancing the effectiveness of performance diagnostics.
FRL-MFPG~\cite{chen2023frl} proposes the Microservice Fault Propagation Graph (MFPG-FC), which combines current microservice dependencies with historical fault data to create a propagation graph that accurately represents fault paths and their impacts.
By integrating historical patterns, FRL-MFPG~\cite{chen2023frl} ensures accurate modeling of fault propagation even as the environment evolves, improving the stability and efficiency of fault diagnosis.
ChangeRCA~\cite{yu2024changerca} integrates service dependency analysis with layered differential analysis to track both the direct and indirect effects of service changes.
By comparing behaviors before and after changes and incorporating historical data, ChangeRCA effectively identifies root causes that might be missed by methods focusing solely on individual service changes. 
This comprehensive approach provides more accurate fault localization and insights into the system’s underlying interactions.


\textit{Tracing anomaly propagation through service dependencies.}
The service dependency is complex and indirect at some times, including asynchronous interactions, caching, and queues. Anomalies can spread via indirect paths, making propagation unpredictable and difficult to model with traditional methods. 
To address this, several approaches focus on modeling these complex interactions and anomaly propagation paths.
MicroRCA~\cite{wu2020microrca} employs attributed graphs to model anomaly propagation paths, capturing both service call relationships and shared host dependencies. 
This comprehensive view allows MicroRCA to focus on critical nodes in the propagation path, narrowing down the scope of root cause analysis and managing complexity effectively.
AutoMAP~\cite{ma2020automap} utilizes an Anomaly Behavior Graph to dynamically generate service correlations and map out intricate propagation routes, including indirect paths through shared resources.
GAMMA~\cite{somashekar2024gamma} addresses bottleneck detection challenges due to complex interactions by employing an attention-based Graph Convolutional Network (GCN). 
This method effectively captures dependencies arising from asynchronous calls, caching, and queues. 
By weighting information from neighboring services, the GCN focuses on critical interactions, enabling accurate and efficient identification of bottlenecks.
TraceAnomaly~\cite{liu2020unsupervised} uses Deep Bayesian Networks to learn normal trace patterns, handling complex dependencies without supervision. 
By creating a unified trace representation that encodes both invocation paths and response times, TraceAnomaly~\cite{liu2020unsupervised} considers the entire trace context, improving anomaly detection accuracy and effectively dealing with intricate service call relationships.
Wu et al.~\cite{wu2020performance} propose a two-stage approach based on a service dependency graph to diagnose performance issues in highly distributed microservice architectures with complex dependencies. 
The first stage identifies potentially problematic services, while the second stage employs an autoencoder to detect specific anomalous metrics related to service abnormalities. 
This approach captures relationships between services and precisely identifies abnormal metrics through reconstruction errors, aiding in pinpointing specific performance bottlenecks.
REASON~\cite{wang2023interdependent} introduces a hierarchical Graph Neural Network (GNN) to capture both intra-level and inter-level non-linear causal relationships in interdependent networks spanning multiple levels. 
This enables accurate modeling of fault propagation across different layers of the system, enhancing the precision of root cause analysis by effectively handling the complexities of multi-layer dependencies.
MonitorRank~\cite{kim2013root} combines a random walk algorithm on the call graph with pseudo-anomaly clustering to handle unreliable call graphs and dynamic dependencies. 
The random walk explores possible root causes without assuming static dependencies, offering flexibility in handling changing system interactions. 
Pseudo-anomaly clustering identifies correlations caused by external factors, supplementing missing information in the call graph.
This combination makes root cause identification more precise and adaptive to the dynamic nature of microservices.
            
\subsubsection{Data Complexity}

In microservice architectures, dealing with the complexity of multidimensional data is another significant challenge. 
These complexities arise from multidimensional data and varying data modalities. 

\paragraph{Multidimensional Data}

Multidimensional data refers to various system-level performance metrics, including CPU usage, memory usage, network input/output, and disk read/write~\cite{nguyen2013fchain}. 
These metrics together represent the system’s overall performance.
Handling these data presents a significant challenge in fault diagnosis due to the complexity of relationships between various metrics.
Several approaches have been proposed to address this challenge by leveraging dependency modeling, dynamic adjustment, and automated learning.

% % MS-RANK 多维度数据

% MS-RANK~\cite{ma2019ms} constructed a dependency graph to model the relationships between multiple performance metrics.
% By leveraging adaptive learning techniques, it dynamically adjusted the weight of each metric to account for changing system states, making the diagnosis more accurate as the dependencies evolved over time. 
% This approach enhanced traditional dependency modeling by explicitly capturing and adapting to the intricate connections among system metrics.

% % Tracecontrast 多维度

% TraceContrast~\cite{zhang2024trace} focused on microservice traces, representing them as sequences of spans with multiple attributes.
% Using contrast sequence pattern mining, it identified rare but critical combinations of attributes associated with anomalies. 
% This method, coupled with spectral analysis, efficiently pinpointed root causes by reducing the dimensionality of trace data, thus tackling the complexity of handling diverse trace attributes.

% % MicroCU多维度

% MicroCU~\cite{jiang2023look} introduced a time-sensitive approach by dividing the anomaly period into short intervals and applying Granger causality tests.
% This allowed for capturing time-varying dependencies between services, rather than relying on static models.
% Through causal unimodalization, it corrected sparse and incomplete metric data, reducing bias in causal inference and enabling more accurate fault propagation analysis.

% % CMMD 多维度

% CMMD~\cite{yan2022cmmd} advanced the field by utilizing Graph Neural Networks (GNNs) to automatically model the complex relationships between different metrics and services. 
% Unlike MS-RANK, which relied on predefined dependency graphs, CMMD learned these dependencies directly from historical data, enabling a more comprehensive analysis across multiple dimensions without manual intervention.
% Additionally, it employed genetic algorithms to efficiently search for anomalous metric combinations, thus enhancing the precision of root cause identification.

% % microscope 多维度数据

% Microscope~\cite{lin2018microscope} simplified the complexity of multidimensional data by capturing real-time service dependencies through system calls. 
% It reduced the number of metrics processed and used statistical methods to handle non-communication dependencies, making causal inference more efficient across diverse system data.

% % fluxrank 多维度数据

% FluxRank~\cite{liu2019fluxrank} tackled the challenge of handling a massive number of diverse metrics. 
% It introduced a lightweight, non-parametric approach combining absolute derivatives and Kernel Density Estimation (KDE) to detect change points.
% FluxRank improved upon previous methods by efficiently identifying significant changes without complex tuning, making real-time failure localization practical.

\textit{Dependency Modeling and Adaptive Learning}
MS-RANK~\cite{ma2019ms} models relationships between multiple performance metrics using a dependency graph. By dynamically adjusting the weight of each metric through adaptive learning, it captures evolving dependencies, leading to more accurate diagnoses.
FChain~\cite{nguyen2013fchain} learns the normal fluctuation patterns of these metrics and identifies abnormal changes. 
FChain then uses these changes, combined with the propagation paths and inter-component dependencies, to accurately pinpoint the faulty component. 
Similar to MS-RANK, it models dependencies between multiple metrics, allowing it to handle complex multidimensional data and improve fault localization without relying on predefined dependency graphs.
CMMD~\cite{yan2022cmmd} takes this further by using Graph Neural Networks (GNNs) to automatically learn complex dependencies between metrics and services from historical data. Unlike MS-RANK, CMMD doesn’t rely on predefined dependency graphs. It also employs genetic algorithms to efficiently identify anomalous metric combinations, improving root cause detection.

\textit{Time Series and Causal Analysis}
MicroCU~\cite{jiang2023look} uses a time-sensitive approach, dividing the anomaly period into intervals and applying Granger causality tests to capture changing dependencies between services. It corrects sparse data through causal unimodalization, reducing bias and improving fault propagation accuracy.
FluxRank~\cite{liu2019fluxrank} addresses the challenge of handling diverse metrics in real-time. Using a non-parametric approach, it combines absolute derivatives and Kernel Density Estimation (KDE) to efficiently detect significant changes, making failure localization more practical without complex tuning.

\textit{Pattern Mining and Dimensionality Reduction}
TraceContrast~\cite{zhang2024trace} focuses on analyzing microservice traces by treating them as sequences with multiple attributes.
It uses contrast sequence pattern mining to detect rare, critical combinations of attributes linked to anomalies and applies spectral analysis to reduce dimensionality for efficient root cause detection.
Microscope~\cite{lin2018microscope} reduces the complexity of multidimensional data by capturing real-time service dependencies through system calls.
Processing fewer metrics and using statistical methods to handle non-communication dependencies, it enhances causal inference across diverse system data.
 
\paragraph{Heterogeneous Data}
As systems became more complex and data more varied, methods needed to adapt to the heterogeneity of data types and system components. 
Researchers developed approaches to effectively integrate different data modalities and address system heterogeneity.

\textit{Data Integration and Representation.}
This category focuses on unifying different data types such as metrics, logs, and traces into a common model.
AutoMAP~\cite{ma2020automap} addresses this by integrating metrics like CPU, memory, and I/O into a unified model through an anomaly behavior graph. 
It dynamically builds relationships between services and uses weighted multi-metric learning to select the most relevant metrics based on historical data, improving diagnostic accuracy.
Similarly, DiagFusion~\cite{zhang2023robust} leverages event embedding techniques like FastText to map logs, metrics, and trace data into a unified vector space. 
By using lightweight pre-processing and representation learning, it effectively integrates diverse data types, utilizing their complementary information to enhance fault diagnosis. 
MULAN~\cite{zheng2024mulan} further advances this approach by using contrastive learning to extract both modality-invariant and modality-specific features from heterogeneous data such as system logs and performance metrics. 
It employs a KPI-aware attention mechanism to fuse these features into a unified causal graph, improving the accuracy of causal relationship modeling.
MicroCause~\cite{meng2020localizing} uses the PCTS algorithm to integrate different types of monitoring data, such as KPIs and metrics, into a unified causal graph.
It fully leverages the time delays and causal relationships between these data types to build an accurate dependency graph. 
Additionally, the TCORW (Temporal Cause Oriented Random Walk) algorithm combines causal relationships, anomaly information (e.g., time of occurrence and severity), and domain-based metric priorities to rank and infer the root causes of failures. 

\textit{Group-based analysis.}
This category organizes similar elements or data types into groups to avoid direct comparisons across heterogeneous elements, thereby improving the precision of anomaly detection.
WinG~\cite{yang2022robust}, for instance, groups elements with similar call characteristics—such as virtual machines, operating systems, and containers—to avoid direct comparisons between these different types of elements. 
It then evaluates anomaly scores within these groups, allowing for more precise detection and root cause localization.

% % Automap 异构数据
% AutoMAP~\cite{ma2020automap} solves the issue of heterogeneous data by introducing an anomaly behaviour graph, integrating different metrics (like CPU, memory, I/O) into a unified model. 
% It dynamically builds relationships between services and uses weighted multi-metric learning to choose the most relevant metrics based on historical data.


% % WinG 异构数据
% While AutoMAP focuses on integrating different types of system metrics into a unified model, WinG~\cite{yang2022robust} groups heterogeneous elements with similar call characteristics to avoid direct comparisons between different types of elements. 
% It then evaluates anomaly scores within these groups, allowing for more precise detection and root cause localization.

% % DiagFusion 异构数据
% DiagFusion~\cite{zhang2023robust} uses event embedding techniques (like FastText) to map logs, metrics, and trace data into a unified vector space, creating a common representation. 
% Through lightweight pre-processing and representation learning, it effectively integrates diverse data, leveraging complementary information to enhance fault diagnosis accuracy.

% % MULAN 异构数据
% MULAN~\cite{zheng2024mulan} extracts both modality-invariant and modality-specific features using contrastive learning to capture unique characteristics from heterogeneous data (like system logs and performance metrics).
% A KPI-aware attention mechanism evaluates each modality’s reliability and fuses them into a unified causal graph for more accurate causal relationship modeling.

% % Fchain 异构
% FChain~\cite{nguyen2013fchain} collects multiple system-level metrics (like CPU, memory, network I/O) to capture normal fluctuation patterns across components.
% It uses an online learning model to predict normal values for each metric and detect abnormal changes, handling different types of system metrics and accurately localizing faults across multi-dimensional data.

% % MicroCause 异构
% MicroCause~\cite{meng2020localizing} solves the challenge of causal learning with heterogeneous data using the PCTS algorithm (Path Condition Time Series). 
% It accurately models causal relationships by leveraging the propagation delays between different monitoring metrics, such as KPIs and system metrics.

In addition to the traditional telemetry data (log, trace, metric), Raccoon~\cite{zhao2023identifying} takes the user-reported incident ticket and the change history as the input, and wants to find which change is the root cause of the incident. They design a causal knowledge representation method at the user-perceived functional level, leveraging fault tree and software product line frameworks, while incorporating multiple knowledge sources and employing a Tree GNN model for causal inference. ChangeRCA~\cite{yu2024changerca} further uses the telemetry data and change history to find the erroneous change.


\subsubsection{Data Path Ambiguity}

In microservice architectures, accurately tracing the flow of data and control across numerous interconnected services is challenging due to data path ambiguity. 
This ambiguity arises from asynchronous communications, lack of global transaction identifiers, interleaved logs from concurrent transactions, and redundant or irrelevant components in service dependency graphs. 
These issues make it difficult to construct precise models of service interactions, hindering effective RCA.
To address this, TraceDiag~\cite{ding2023tracediag} proposes a framework that employs reinforcement learning (RL) to automatically learn optimal pruning strategies. 
By learning from historical data, RL effectively identifies and removes redundant components, enhancing RCA efficiency and reducing manual intervention. 
This adaptive approach balances the pruning process to prevent both over-pruning and under-pruning, ensuring that essential components are retained while irrelevant ones are discarded.

Another significant challenge is \textit{dealing with ambiguities in call data within complex, interdependent microservices}.
Even with a well-constructed, ambiguity-free call graph, incorrect traversal and interpretation can lead to inaccurate root cause identification.
To tackle this issue, CMDiagnostor~\cite{yu2023cmdiagnostor} integrates the AmSitor algorithm, which uses a regression-based method to accurately determine associations between upstream and downstream calls, particularly in ambiguous situations.
AmSitor models the relationship between upstream and downstream traffic using linear regression, estimating weights that represent the expected number of downstream calls per upstream call. 
By filtering out connections with low or negligible coefficients and iteratively applying regression across different time slices of call data, it retains only those upstream-downstream pairs that consistently show strong connections. 
This results in a clear and accurate call graph.
Building upon this, CMDiagnostor employs a series of pruning strategies—such as AmSitor-based, Metric Similarity-based, and Anomaly Detection-based Pruning—to effectively navigate the call graph. 
These strategies filter out false positives and focus on the most relevant paths, ensuring that the root cause localization process remains precise and effective, even in large-scale systems with complex interdependencies.

Moreover, instead of using a snapshot of the entire system for incident detection, traditional methods often \textit{neglect the importance of issue extraction}. 
This approach can lead to outdated analysis, high false alert rates, and difficulties in integrating information from various sources.
GIED\cite{he2022graph} addresses this by automatically extracting the issue impact topology early in incident management, considering both symptoms and affected services.
By focusing on the specific parts of the system impacted by an issue, GIED allows for more accurate incident detection and efficient root cause localization. It utilizes a Graph Neural Network (GNN)-based model and the PageRank\cite{brin1998anatomy} algorithm to analyze the extracted topology, improving detection accuracy and reducing false positives.

Finally, in scenarios without transaction IDs, \textit{extracting control flow graphs from multi-threaded logs} presents a challenge due to interleaved logs from different threads. 
This interleaving makes it difficult to separate actual execution paths from noise, leading to confusion where logs from different transactions may appear falsely related.
To overcome this, Jia et al.~\cite{jia2017approach} propose a two-stage edge mining algorithm. The first stage identifies frequent successor groups—logs that frequently occur close together in time—to uncover potential true relationships. The second stage refines these groups to find immediate successors, removing redundant and incorrect links. This approach leverages statistical associations between log entries, capturing real relationships within execution paths and reducing confusion caused by interleaved logs. By broadening the search for potential connections and then narrowing it down to the most relevant ones, the method effectively minimizes noise and reconstructs accurate control flow graphs.



\subsubsection{Scarcity of Incident-related Data}

The lack of high-quality incident-related data can lead to several issues in both supervised and unsupervised RCA methods. 
In unsupervised approaches, noise in the data often poses a significant challenge, as normal patterns can be misinterpreted as anomalies due to their variability, which reduces the precision of anomaly detection.
In supervised methods, an imbalance between normal and abnormal data leads to models favoring the more common normal data, which results in missed anomalies or false alarms. 
This imbalance can reduce the overall accuracy of both anomaly detection and root cause localization, making it difficult to effectively diagnose incidents in complex systems.

Sample scarcity is a challenge for root cause analysis in cloud computing platforms, as there are often too few failure events to train effective models.
To address this, CloudRCA~\cite{zhang2021cloudrca} uses cross-platform transfer learning, sharing data between Alibaba’s different cloud platforms (MaxCompute, Realtime Compute, Hologres), especially for common modules like hosts and networks. By pooling data from these platforms, the method compensates for the lack of data on individual platforms, improving the model’s ability to generalise and accurately identify new failures. This approach is especially helpful as cloud-native architectures become more unified

One of the major challenges MicroCBR~\cite{liu2022microcbr} faces is the lack of incident-related data. In microservice environments, data like logs, metrics, and traces can be incomplete due to deployment configurations, security constraints, or performance requirements. This missing data makes it difficult for traditional diagnostic methods, which often rely on specific homogeneous data types, to effectively identify faults.
To address this issue, MicroCBR~\cite{liu2022microcbr} integrates heterogeneous data sources, including metrics, logs, traces, and command outputs. 
This approach improves data coverage by allowing available sources to fill in for missing data. Command data, in particular, serves as a customizable post-incident source, providing additional insights when other types are unavailable. 
By combining multiple data types, MicroCBR enhances system diagnosis, ensuring that even with incomplete data, useful insights can still be obtained, making the process more robust and effective.

In Microrank~\cite{yu2021microrank}, the imbalance in the coverage of normal and abnormal traces in the data makes traditional spectrum-based methods less effective, as some requests frequently cover the same service instances while others do not.
To address this imbalance, MicroRank~\cite{yu2021microrank} incorporates a personalized PageRank algorithm that assigns different weights to traces based on their ability to localize root causes. The algorithm considers both the scope of the traces (i.e., how many service instances they cover) and the frequency of different types of traces. 
By doing so, MicroRank~\cite{yu2021microrank} balances the influence of frequently and infrequently occurring traces, ensuring that the spectrum analysis accurately reflects the importance of each trace in diagnosing root causes. 
This approach enhances the precision of root cause localization by mitigating the bias introduced by unbalanced trace coverage.

Diagfusion~\cite{zhang2023robust} uses a data augmentation mechanism that generates more samples for rare failure types by randomly selecting and modifying events from the original data. This approach helps balance the training data, allowing the model to better learn the characteristics of all failure types and improving its ability to diagnose rare failures accurately.
Additionally, SparseRCA~\cite{yao2024sparserca} addresses the challenge of not being able to fully obtain the fault propagation information, such as call relationships in sparse trace scenarios. It analyzes anomalies in exclusive latency at the span level to directly estimate the probability of a microservice being the root cause, addressing the challenge of insufficient fault propagation information in sparse trace scenarios. By leveraging pattern-based latency distribution modeling and pattern prediction, SparseRCA demonstrates robust generalization capabilities to handle dynamic updates and unseen trace structures. 


\subsubsection{Difficulty in Obtaining Labeled Data}

Obtaining labeled data for RCA is inherently challenging, since there are no ground truth labels for RCA in the industry, only if a failure is detected and resolved by the SRE, and the telemetry data are stored for post-mortem analysis. 
Thus, unsupervised methods are important in industry because they reduce the human effort for labeling data, and the need for storing historical telemetry data of a failure. 
Given the inherent difficulty of obtaining labeled data, various unsupervised methods have been proposed to address this challenge from different perspectives, such as statistical analysis~\cite{shan2019diagnosis, pham2024baro}, causal inference~\cite{gan2021sage, xie2024microservice}, and pattern mining~\cite{zhang2021onion, yu2023nezha, gan2023sleuth}. 


% 基本所有无监督的都是构建一个图

% $\varepsilon$-Diagnosis 

% Both Sage~\cite{gan2021sage} 



\textit{Statistical Methods.} 
Statistical methods primarily rely on detecting changes in data distributions, often without the need for pre-labeled datasets or prior assumptions about system behaviors. 
These methods are particularly useful in real-time settings where timely anomaly detection is crucial.
% e-Diagnosis'19
% $\varepsilon$-Diagnosis~\cite{shan2019diagnosis}
Instead of relying on labeled data, $\epsilon$-Diagnosis~\cite{shan2019diagnosis} uses unsupervised two-sample hypothesis testing and time series similarity analysis to identify root causes.
By comparing abnormal and normal samples, the algorithm efficiently detects significant changes in metrics, providing a practical solution to the labeled data challenge, particularly in real-time diagnosis scenarios.
BARO~\cite{pham2024baro} builds on this idea by employing a more sophisticated approach for multivariate time series. 
It incorporates Multivariate Bayesian Online Change Point Detection to effectively detect anomalies in complex time series data without relying on labeled datasets. 
Additionally, BARO uses a nonparametric hypothesis testing method, RobustScorer, which is robust to inaccuracies in anomaly detection and does not require pre-labeled data.

% MicroRank~\cite{yu2021microrank}


\textit{Causal Inference-Based Methods.} 
In contrast to statistical methods, causal inference-based approaches aim to uncover the underlying causal relationships between variables, offering a deeper understanding of how system anomalies emerge from complex interdependencies. These methods are particularly powerful when dealing with latent variables and missing information.
% Causal inference~\cite{yao2021survey} is widely used in 
% Sage~\cite{gan2021sage}
Sage~\cite{gan2021sage} utilizes Conditional Variational Autoencoders (CVAE) to model the distribution of latent variables from historical tracing data collected by cloud monitoring systems.
By generating counterfactual scenarios, Sage simulates how different conditions might affect system performance, allowing it to infer the root causes of QoS violations without relying on pre-labeled data. 
This process involves using the observed data to train the model and then applying it to generate hypothetical cases where potential issues could arise, thus enabling the system to diagnose problems based on the learned patterns from historical data.
% CIRCA~\cite{li2022causal}
Unlike Sage~\cite{gan2021sage}, CIRCA~\cite{li2022causal} addresses the challenge of limited labeled data by constructing a CBN and using regression techniques to handle incomplete fault data distributions. 
CIRCA~\cite{li2022causal} adjusts anomaly scores without relying on labeled data, making it effective in scenarios with scarce labeled information. 
This model focuses more on refining anomaly scores based on partial data, which complements Sage’s focus on generating counterfactuals for hypothesis testing.
% LatentScope~\cite{xie2024microservice}
LatentScope~\cite{xie2024microservice} addresses the difficulty by introducing unsupervised methods like the Regression-based Latent-space Intervention Recognition (RLIR) algorithm and its enhancement, LatentRegressor. 
Unlike traditional supervised models that require labeled data, RLIR operates in a latent space, allowing it to infer the status of unobservable variables without the need for labeled data. 
LatentRegressor further refines this process by using ridge regression, which is more robust to noise, reducing computational overhead and enhancing accuracy in real-world applications. 


\textit{Pattern Mining-Based Methods.} 
Unlike statistical or causal inference-based approaches, pattern mining methods focus on discovering commonalities and deviations within large datasets. 
These methods directly identify patterns associated with failures through automated clustering and comparison, reducing reliance on labeled data.
% Onion
In cloud system log analysis, the large volume and complexity of logs make manual labeling of incident-indicating logs time-consuming and error-prone.
By leveraging automated clustering techniques, Onion~\cite{zhang2021onion} groups similar logs into “log cliques” and uses contrast analysis to compare logs from anomalous servers with those from normal servers, effectively identifying incident-indicating logs.
This approach avoids the need for extensive manual labeling and, compared to traditional template-based log analysis methods, is more adaptable and maintains high accuracy and efficiency even when labeled data is incomplete.
% Nezha~\cite{yu2023nezha}
Nezha~\cite{yu2023nezha} takes this idea further by analyzing multi-modal data, such as logs, traces, and metrics, before and after faults occur.
It constructs an event graph and compares execution patterns to detect anomalies. 
Nezha~\cite{yu2023nezha} automatically pinpoints potential root causes by detecting patterns that deviate from expected paths, thereby reducing reliance on manual labeling and handling larger, more complex datasets.
% Sleuth~\cite{gan2023sleuth}
Sleuth~\cite{gan2023sleuth} enhances pattern mining techniques by adopting an unsupervised learning approach that leverages a GNN to model causal relationships between services in a microservices architecture.
Then it generates counterfactual queries to identify the root causes of anomalies. 
This approach allows Sleuth to operate effectively without any labeled data. 
Moreover, Sleuth’s design includes few-shot learning capabilities, ensuring it remains highly adaptable and generalizable across different microservice applications, even with minimal or no labeled data available.




\subsection{ACCURACY OF ANOMALY DETECTION} \label{sec:anomalydetection}
In large-scale microservice systems, accurately detecting anomalies presents several key challenges: \textit{parameter sensitivity in statistical methods}, \textit{complex service dependencies}, and \textit{diverse anomaly types}. 
Addressing these challenges is crucial for ensuring that anomaly detection can effectively support root cause analysis (RCA). 
Below, we examine how different methods tackle these issues.

\textit{Parameter Tuning and Data Limitations.} 
Firstly, existing methods like Kernel Density Estimation (KDE) and $epsilon$-statistical tests often struggle with \textit{parameter tuning and data limitations}, leading to inaccurate anomaly detection. 
PatternMatcher~\cite{wu2021identifying} addresses this by using a two-sample hypothesis test for coarse-grained anomaly detection, which compares data distributions before and during anomalies. This method reduces parameter sensitivity and improves detection reliability by avoiding the complex tuning required in KDE.

\textit{Complex Dependencies and Diverse Anomaly Types}
In addition, the \textit{complex dependencies and diverse anomaly types} in microservices create further challenges. 
MicroHECL~\cite{liu2021microhecl} offers a solution by combining machine learning and statistical methods to handle different anomaly types more effectively.
It uses OC-SVM for performance anomalies, Random Forest for reliability anomalies, and the 3-sigma rule for traffic anomalies, ensuring more precise detection across multiple anomaly types.

\textit{Complex Dependencies in Multivariate Time Series.}
Eadro~\cite{lee2023eadro} takes a step further by integrating anomaly detection and root cause localization in an end-to-end manner, using multimodal learning to create a unified system representation from logs, KPIs, and traces.
By jointly optimizing both tasks, Eadro enhances detection and localization accuracy.
Based on previous study \cite{bai2018empirical}, Eadro relies on 1D dilated causal convolution (DCC) \cite{lea2016temporal} layer to handle \textit{complex dependencies in multivariate time series}. 
In addition, BARO~\cite{pham2024baro} addresses it by introducing Multivariate Bayesian Online Change Point Detection (BOCPD), which models dependency structures more accurately, improving anomaly detection in complex systems.
Its RobustScorer method ranks root causes based on data distribution changes, making root cause analysis less sensitive to detection timing.







==> chapters/legacy_output.tex <==
\section{CHALLENGES OF OUTPUT} 

Root Cause Analysis (RCA) is designed to equip Site Reliability Engineers (SREs) with the ability to quickly and accurately identify both the “what” and the “how” of an anomaly.
To be truly effective, the output of RCA must be fine-grained and interpretable. 
A \textbf{fine-grained} output means isolating the ultimate root cause, enabling SREs to address it, thereby directly resolving all associated abnormal behaviors. \textbf{Interpretability} ensures that these results are easy to understand, reducing the time SREs spend on verification.
Therefore, the challenges of RCA outputs can be distilled into two key aspects: producing highly detailed results and ensuring those results are easy to understand.


\subsection{DIFFERENT GRANULARITY OF ROOT CAUSE}\label{sec:granularity}

In the literature, various methods yield root causes at differing levels of granularity. To fully grasp this concept, it’s important to understand that the granularity of identified root causes is closely tied to the granularity of the input data. Simply adding more fine-grained observation data enables the inference of more detailed root causes. To illustrate this, we use an example from the TrainTicket case~\cite{zhou2018fault} to demonstrate the hierarchical nature of root cause granularities. From this view, we can comprehensively understand the relationships between the input data and the output result.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/rootcauses.pdf}
    \caption{Multi-level root causes}
    \label{fig:rootcaues}
\end{figure}



Root causes can be categorized into three primary levels: service level, resource level, and component level, with each successive level providing finer granularity. 
Each level is derived from the observation space, where finer-grained levels generally encompass the results from coarser-grained levels. 
For example, in Fig.~\ref{fig:rootcaues} the assurance service has logical dependencies on the preserve service, and both services are deployed on Kubernetes.
Drilling down further, within a specific resource (such as a container), more detailed resources and attributes can be observed, like the CPU, Memory usage.
Depending on the scenario, the root cause could be at any of these levels~\footnote{In industry practice, the root causes usually are combinations of these levels, composing which service, which resource, and which component}. 
For instance, if the SRE team needs to identify which team to contact, the service-level root cause might suffice. On the other hand, if the development team is tasked with fixing the issue, they may require more granular information, such as the root causes related to configuration changes or code changes.


\subsubsection{At the service level}
The root cause pertains to identifying which service is responsible for the observed anomaly (often indicated by a violation of Service Level Objectives, or SLOs)~\cite{wang2018cloudranger,ma2020self,ma2020automap,ma2021servicerank,wang2023root,zhou2019latent,liu2021microhecl,liu2020unsupervised,li2021practical,yu2023tracerank,gan2021sage,lee2023eadro,zheng2024mulan,yu2023cmdiagnostor,harsh2023murphy,yu2021microrank,yan2022cmmd,wu2020microrca,kim2013root,lin2018microscope,ding2023tracediag,somashekar2024gamma,ikram2022root,ma2019ms,li2022microsketch,yang2023tracenet,liu2019fluxrank,nguyen2013fchain,li2022swisslog,jia2017approach}. This helps SREs narrow down the search space from potentially thousands of services to just a few. For example, the system in Ant Group consists 3000+ microservices running on over 1 million virtual containers~\cite{wu2023empirical}. 
Resolving the root cause among these services is relatively difficult. 
At this level, the provided telemetry data (input) sometimes includes only service-specific metrics, such as CPU usage, service logs, and inter-service calling traces. 
Although helpful, the result of the RCA is too fine-grained, since the possible failure search space is still large within a single service. 
The underlined reason may be the model might not leverage fine-grained data, thereby limiting its ability to pinpoint the exact root cause. It can only determine which service is responsible for the current issue.

\subsubsection{At the resource level} Multiple runtime resources are managed in the cloud-native environment, like deployment, stateful set, and pod. 
Some approaches~\cite{wang2023interdependent,zhang2023robust,wang2023incremental,gan2023sleuth,he2022graph,shan2019diagnosis,pan2021faster,yang2022robust,cai2021modelcoder,sauvanaud2016anomaly} pinpoint the specific resource, such as a pod or container, that is the root cause of the failure. 
This provides SREs with a more direct focus for further investigation. At this level, the ability to identify the root cause is largely due to the availability of more granular data, including metrics and logs specific to individual pods, containers, and hosts. 
By leveraging this fine-grained information, the methodologies can correlate anomalies directly with specific resources, rather than just higher-level services. 
This allows for a more precise diagnosis, facilitating quicker and more targeted remediation efforts. 
Consequently, the identification at the resource level not only reduces the search space further but also enhances the accuracy of the troubleshooting process, ultimately leading to more efficient incident resolution in cloud-native environments.

\subsubsection{At the component level} Where methods~\cite{li2022actionable,yu2024changerca,li2022causal,pham2024baro,zhang2024illuminating,wang2021groot,yao2024chain,meng2020localizing,chen2014causeinfer,zhang2021onion,kong2024enhancing,hou2021Pdiagnose,guo2020graph,jiang2023look,murali2021scalable,wang2015methodology,jayathilaka2017performance,rosenberg2020spectrum,thalheim2017sieve,zhang2024fault,wang2020root,jeyakumar2019explainit,lin2018facgraph,hu2022ts,nie2016mining,lu2022generic,mariani2018localizing,chen2023frl,wu2020performance,sharma2013cloudpd,sui2023logkg,amar2019mining,he2018identifying,lu2017log,ikeuchi2018root} the inner component within some service or resource at fault, e.g., which lines of code, which operation, or which change event is the root cause. 
This level of granularity is achievable due to the availability of highly detailed observational data. 
For instance, logs may contain specific code snippets, traces might include function calls and attributes such as OS versions and the tools used for data collection, and metrics could detail the exact objects being monitored. 
We also categorize methods that identify specific telemetry data, such as a particular log~\cite{zhang2021onion} or a detailed metric, as the root cause at the component level. 
This is because such telemetry data inherently includes information about the corresponding component, such as file names, line numbers for logs, or the specific component associated with a metric or trace. 
By utilizing such fine-grained inputs, these approaches can output similarly detailed diagnoses, pinpointing the exact component responsible for the issue. 
This capability is critical for SREs and developers as it not only identifies the problematic component but also provides actionable insights that can be directly linked to the codebase or configuration settings. 
As a result, the troubleshooting process is accelerated, enabling more effective debugging and quicker resolution of incidents at a micro-level within the system.

\subsubsection{At Multi-dimension level} There could be multiple output levels at the same time. 
In this approach, the algorithm considers the characteristics of the input data to identify root causes across various levels simultaneously, including service, resource, and component levels~\cite{yu2023nezha,zhang2024trace,xie2024microservice,gu2023trinityrcl,zhang2021halo,zhang2021cloudrca,liu2022microcbr}. 
This level of analysis is highly adaptive, allowing it to provide the most context-appropriate diagnosis depending on the nature of the anomaly and the data available. 
For instance, an issue might be traced back to a specific service at the service level, while concurrently identifying a particular pod at the resource level and pinpointing a faulty code snippet at the component level. 
This multi-dimensional output is particularly valuable in complex, cloud-native environments where issues often span multiple layers of the infrastructure.
By offering a comprehensive view that integrates insights from multiple levels, this approach empowers SREs and developers to address problems more holistically, ensuring that all potential root causes are considered and that remediation efforts are both targeted and effective. 
For example, Nezha~\cite{yu2023nezha} can localize three types of output, i.e., service, code region, and telemetry type; TrinityRCL~\cite{gu2023trinityrcl} can output application, service, host, metric and code level root causes.
GAMMA~\cite{somashekar2024gamma} addresses the challenge of multiple bottlenecks in microservices architecture (MSA), which can occur independently, dependently, or in a cascading manner, a scenario that has been largely overlooked by existing research that mainly deals with single bottlenecks.

Through these multi-level outputs, it becomes clear that the granularity of the output is fundamentally determined by two key factors: \textbf{the utilization rate of the input data} (which varies depending on how different models process the data) and \textbf{the granularity of the input data itself}. 
Regardless of the model’s effectiveness in utilizing data, the finest granularity of the output is limited by the detail present in the input. 
At best, we can pinpoint the smallest component within the observed data as the root cause of the anomaly, or we might determine that the root cause lies outside the current observation space~\cite{xie2024microservice}. 
Therefore, achieving finer granularity in root cause analysis hinges on two main challenges: enhancing the utilization of input data and increasing the granularity of the observed data. 
These aspects have been discussed in detail in Section~\ref{sec:input}.


\subsection{INTERPRETABLE LOCALIZATION RESULTS}
 
%讨论下对于root cause的自然语言解释。例如利用历史数据解释等等。
% explainit
% 

Interpretability is another crucial objective in root cause analysis, as it allows Site Reliability Engineers (SREs) to rapidly comprehend what transpired within the running service, why anomalies occurred, and how to resolve them. 
Similar to the granularity of root causes, interpretability can be classified into various levels, ranging from identifying a \textit{single root cause} to constructing a \textit{fault propagation graph}. 
The single root cause approach assumes there is only one underlying cause, while the fault propagation graph illustrates the dependencies and causal relationships among multiple root causes. 
Between these two extremes, intermediate levels exist, such as identifying \textit{multiple root causes} or tracing a \textit{fault propagation chain}.
Additionally, we will also discuss the methods that output \textit{explanations} of root causes/incidents.

\subsubsection{Single Root Cause} This level is suited for models designed to identify only one root cause, without considering scenarios involving interactions between multiple root causes. The output is typically a ranked list of suspected root causes, with only one being the ground truth. For instance, although Eadro~\cite{lee2023eadro}, BARO~\cite{pham2024baro}, and related works~\cite{meng2020localizing,yu2024changerca,gu2023trinityrcl,zhou2019latent,ma2020automap,wang2018cloudranger,ma2019ms,ma2020self,ma2021servicerank,liu2021microhecl,liu2020unsupervised,wang2015methodology,jayathilaka2017performance,rosenberg2020spectrum,thalheim2017sieve,li2022causal,wang2023incremental,chen2014causeinfer,zhang2023robust,pan2021faster,he2022graph,zhang2021halo,xie2024microservice,zheng2024mulan,lin2018microscope,murali2021scalable,kim2013root,zhang2021onion,hou2021Pdiagnose,gan2021sage,gan2023sleuth,kong2024enhancing,zhang2024fault,zhang2024trace,ding2023tracediag,li2021practical,ma2020diagnosing,liu2022microcbr,zhang2021cloudrca,wang2020root,li2022microsketch,yang2023tracenet,yang2022robust,cai2021modelcoder,jeyakumar2019explainit,lin2018facgraph,hu2022ts,sauvanaud2016anomaly,nie2016mining,lu2022generic,mariani2018localizing,chen2023frl,wu2020performance,sharma2013cloudpd,liu2019fluxrank,nguyen2013fchain,sui2023logkg,li2022swisslog,jia2017approach,amar2019mining,he2018identifying,lu2017log,ikeuchi2018root,yan2022cmmd} produce outputs at varying levels of granularity, as discussed in Section~\ref{sec:granularity}, they all focus on identifying a single root cause, implying that only one root cause exists within the current observation space. However, in reality, multiple root causes can coexist—such as a configuration change being the root cause and a surge in requests acting as the trigger described in Section~\ref{sec:preliminaries}. In such cases, the absence of the trigger would mean the root cause might not lead to the observed anomaly. Thus, the current models may overlook complex scenarios where multiple root causes work together to produce the observed issue.


% \subsubsection{Multiple Root Causes} 

% At this level, the model recognizes that real-world scenarios often involve multiple interacting root causes~\cite{somashekar2024gamma,ikram2022root}. It generates a list of potential root causes reflecting this complexity, providing a more comprehensive understanding of the issue than single root cause approaches. For example, GAMMA~\cite{somashekar2024gamma} addresses the challenge of multiple bottlenecks in microservices architecture (MSA), which can occur independently, dependently, or in a cascading manner, a scenario that has been largely overlooked by existing research that mainly deals with single bottlenecks.
% However, while these methods account for multiple root causes, they typically do not address the interactions and dependencies between them. In other words, they identify the possible root causes but do not explain how these root causes interact to create the current situation. This limitation leaves a gap in understanding the causal relationships that lead to the observed problem, which is crucial for effective remediation and prevention strategies.


\subsubsection{Fault Propagation Graph} 

The fault propagation graph could be considered as the most interpretable illustration of the root causes since it contains the single root causes as the nodes and the possible propagation path as the edges. In this graph, the node root cause can be multi-dimensional as mentioned in the previous section, including the service level, resource level, and component level.
This graph-based approach offers the most detailed and comprehensive explanation of how the current anomalies have occurred by capturing the intricate relationships and dependencies between multiple root causes. However, achieving this level of detail is challenging due to several factors.

\textit{(1) Obtaining accurate ground truth is difficult}, as SREs and other operational staff may have varying or incomplete understandings of the incidents, leading to inconsistent or incorrect interpretations. 

\textit{(2) There is a lack of standardized evaluation metrics for fault propagation graphs~\cite{zhang2024illuminating}}, making it hard to compare methods or validate their effectiveness at this level. These challenges have limited the development and adoption of strategies that fully meet the definition of a fault propagation graph.

As far as we know, ServerRCA~\cite{shi2023serverrca} is the only method that formally claims that they output a fault propagation chain, indicating how the fault propagates from the ultimate root cause to the intermediate root cause. However, due to the aforementioned limitations, it still uses the $HR@K$ metric to evaluate the fault propagation chain, where the root node of the true fault propagation chain is the root cause.
Nevertheless, many existing methods do maintain an internal graph structure to represent the spread of anomalies~\cite{yao2024chain,zhang2024illuminating,harsh2023murphy,yu2023nezha,jiang2023look,wang2021groot,wang2023interdependent,yu2023cmdiagnostor,yu2021microrank,li2022actionable,ma2020automap,wang2018cloudranger,wang2023root,ma2020self,liu2021microhecl,brandon2020graph,murali2021scalable,wang2015methodology,li2022causal,wang2023incremental,chen2014causeinfer,pan2021faster,guo2020graph,wu2020microrca,lin2018microscope,kong2024enhancing,zhang2024trace}, even if their final output is simplified to a root cause list. To acknowledge the significance of these methods, we discuss those that incorporate an internal fault propagation graph. Despite the mentioned challenges, these methods often revert to producing a ranked list of root causes, as the complexity of fully utilizing the graph structure remains an unresolved challenge in the field.

Three notable works focusing on fault propagation paths are Groot~\cite{wang2021groot}, Chain-of-Event~\cite{yao2024chain}, and GrayScope~\cite{zhang2024illuminating}. Specifically, Groot~\cite{wang2021groot} employs a user interface to visually display the propagation path of anomalies, making it easier for SREs to verify root causes. Chain-of-Event~\cite{yao2024chain} addresses three key questions: how different events influence each other, how the model arrives at its conclusions, and how suspicious a given event chain appears to SREs. These questions help provide a detailed illustration of the incident, aiding SREs in understanding the fault propagation. Since there is no standard definition for evaluating the precision of failure propagation paths, GrayScope~\cite{zhang2024illuminating} relies on human evaluation to assess their method's effectiveness.
Other works like ~\cite{harsh2023murphy,yu2023nezha,jiang2023look,wang2023interdependent,yu2023cmdiagnostor,yu2021microrank,li2022actionable,wang2018cloudranger,ma2020self,liu2021microhecl} internally maintained a fault propagation graph, but they did not address or partially address the interpretability issue in terms of fault propagation graph.

There are also works providing the graph similarity metrics. For example, Brandón et al.~\cite{brandon2020graph} propose a graph similarity engine that is used to detect the anomalies in the graph. By composing the graph elements(node, edge, context), the graph similarity is calculated to detect the anomaly. However, they did not emphasize this point, which is possible to be used for evaluating the interpretability issue.



\subsubsection{Explanation of Root Cause/Incident Ticket}


The field of root cause and incident explanation can be divided into two main parts. The first involves explaining root cause candidates, including identifying the types of root causes and determining the specific category of potential faults. This is typically achieved by leveraging historical incident databases, which store past error data along with human-provided explanations. By matching new cases with similar past incidents, models can offer SREs relevant insights and references.
The second part, distinct from traditional root cause analysis (RCA) methods, focuses on incident tickets as input. This emerging area of research, which gained traction around 2023, has been largely driven by advances in large language models (LLMs). LLMs enable the provision of detailed incident explanations within operational processes, filtering out irrelevant issues and compiling pertinent information. In our reviewed literature, five works~\cite{ahmed2023recommending,zhang2024automated,zhang2024lm,chen2024automatic} have explored this area, highlighting the potential of LLMs in enhancing incident management and explanation.

Failure type is the most frequently used explanation, typically the action/symptom of the component or resources. Combining output multi-level root causes and the corresponding possible failure types can provide more interpretable results for SREs.
For example, Déjàvu~\cite{li2022actionable} considers bad requests, unavailable third-party services, failed disks, slow SQL queries, etc. as their failure types. MEPFL~\cite{zhou2019latent} also categorizes the failure categories into configuration-related, resource-related instance-related, and interaction-related. Their implementations usually contain using the previous known failure database to retrieve similar cases~\cite{li2022actionable,ma2020automap,sui2023logkg}. The most common failure types are discussed by numerous studies and surveys~\cite{ganatra2023detection,jiang2020mitigate,gunawi2014bugs,liu2019bugs,zhao2023manage,wu2023empirical,ghosh2022fight,chen2020incidental,gunawi2016does}, thus we did not extend it.



Unlike other works we introduced in previous sections, the input of the following papers are all incident descriptions, like incident tickets.
These data are usually described in natural language. Thus, it is suitable to use the Large Language Model to interpret the potential root cause behind the incident.
ICSE'23~\cite{ahmed2023recommending} did a rigorous study at Microsoft, on more than 40,000 incidents and compared several large language models in zero-shot, fine-tuned, and multi-task settings using semantic and lexical metrics.
RCACopilot~\cite{chen2024automatic} is a system that leverages historical incident data and predefined rules to match incoming incidents with the most appropriate handlers based on the type of alert. For instance, if an alert pertains to a database connection issue, the system automatically assigns it to a database administrator. By integrating this capability, RCACopilot enhances the efficiency of incident resolution by reducing the manual effort traditionally required to investigate logs and trace data sources. Moreover, RCACopilot goes a step further by generating explanatory narratives for each incident. These narratives provide engineers with a comprehensive understanding of the incident, including context, the identified root cause, and recommended actions for resolution. This capability is crucial in helping on-call engineers quickly grasp the situation and respond effectively.
ICLRCA~\cite{zhang2024automated} uses a standard RAG and In-context-learning pipeline to retrieve the possible root cause of the provided incident. Specifically, it involves collecting and cleaning incident data, summarizing the incidents using GPT-3.5-turbo, and creating embedding vectors with a sentence transformer model. These embeddings are used to build a retrieval index with the Faiss library for efficient similarity searches. When a new incident occurs, relevant examples are retrieved from the index and included in a prompt provided to a large language model (e.g., GPT-4), which then generates the root cause analysis based on the new incident description and the retrieved in-context examples.
To generate calibrated confidence scores, LM-PACE~\cite{zhang2024lm} involves prompting the model in two distinct stages. In the first stage, the model quantifies the strength of evidence derived from historical incidents, allowing for an equitable assessment of the current incident. Subsequently, the second stage prompts the model to evaluate the candidate root cause produced by the root-cause predictor, utilizing the same set of references. A transformation is then applied to a validation set to estimate the confidence level based on the two scores generated from the prompting stages. 
% Additionally, to address the challenges of limited historical data and evolving systems in root cause localization, OCRCL~\cite{huang2024ocrcl} not only integrates incident tickets, but also service text semantics, and static service dependency structures, employing online incremental learning to incorporate historical incident information and enhance model accuracy. By leveraging contrastive learning, OCRCL~\cite{huang2024ocrcl} augments incident tickets to improve the model's ability to link incidents with root causes. 
While this area shows great promise, it is still in its early stages, and further research is needed to refine these methods, improve their accuracy, and expand their applicability to a broader range of incidents.


==> chapters/test_01.tex <==
%ServiceRank
% 关闭容器 - Resources
% DoS - Input

%Roots
% 增加服务响应时间 - Input

%AutoMAP 
% 关闭容器 - Resources
% DoS - Input

%TraceAnomaly
% 增加服务响应时间 - Input
% 通过移除微服务节点来模拟调用路径的异常 - Service Dependency

%TraceRCA
% 应用程序错误 - Code
% CPU资源耗尽；网络延迟 - Resources

%Microscope
% 容器挂起；CPU资源耗尽；网络延迟 - Resources

%Graph-based-root-cause analysis
% 带宽限制；网络延迟；错误的负载均衡；端点压力；系统资源压力 - Resources

%MicroRCA
% 网络延迟；cpu 资源耗尽；内存泄漏 - Resources

%CloudRanger
% 关闭 service host - infra dependency

%CauseInfer
% Resources
% Code

%PDiagnose
% AIOps challenge

%RCSF
% 服务器攻击 - Input
% 流量负载迁移 - Resources or Service Dependency

%RCD
% cpu 资源耗尽；内存泄漏 - Resources

%MEPFL
% 多实例故障 - services dependency
% 配置故障 - configuration
% 异步交互故障 - services dependency

%Sage
% resources contention(CPU ..) - Resources
% 软件缺陷：包括并发缺陷、线程或连接池不足等问题，这类故障更偏向于逻辑层面，可能导致服务无响应或性能瓶颈 - code

%Dycause
% 增加内部服务的延迟 - Services dependency

%LatentScope
% 第三方服务错误，内部服务运行时错误，数据库服务中断 - Services dependency
% 配置变更 - config

%ChangeRCA
% Defective Backend Change - code
% Defective Config Change - config
% xxx - resources

%CIRCA
% 这个需要再看看

%GAMMA
% xx - resources

%HRLHF
% 后端服务的内部延迟 - services dependency

%CMMD
% 这个也得再看看

%GIED
% xx - resources

%BARO
% xx - resources

%REASON
% xx - resources

%GrayScope
% xx - resources

%MicroRank
% xx - resources

%Murphy
% xx - resources

%TraceContrast
% xx - resources

%Sleuth
% CPU，内存，网络xxx，分别在容器，pod 和节点级别注入- resources

%SpanGraph
% 多实例故障 - services dependency
% 配置故障 - configuration
% 异步交互故障 - services dependency

%Nezha
% CPu 竞争，网络堵塞 - resources
% 错误返回，异常代码缺陷 - code

%Eadro
% CPU 资源耗尽，网络延迟，网络包丢失 - resources

%Diagfusion
% System Failure - OS
% service failure - services

%SpanGraph
% 多实例故障 - services dependency; 归类为 hard to determine
% 配置故障 - configuration
% 异步交互故障 - services dependency
% 代码逻辑问题 - code

%Onion
% resource contention - resources
% 操作员错误配置引起的连接问题 - operations
% 软件环境依赖冲突 - Runtime Env.

%ICSOC20
% cpu资源耗尽；内存泄漏 - resources

%Fchain
% xx - resources
% 代码逻辑问题 - code

%FRL-MFPG
% resources contention; CPU 资源耗尽；网络延迟 - resources
% 高请求负载 - user request

%LOUD
% resources contention; CPU 资源耗尽；网络包丢失 - resources

%TS-InvarNet
% resources contention; CPU 资源耗尽；网络包丢失 - resources

%ExplainIt
% 网络包丢失 - resources

%CloudPD
% resource contention - resources
% 配置故障 - config

%DBSherlock
% xx - resources
% 低效查询 - user request
% 不良物理设计 - Infrastructure dependency

%FPDB
% 包含性故障 - services
% 传播性故障 - services dependency

%TraceNet
% 网络相关 - resources

%MicroSketch
% 网络故障，CPU 故障，硬盘读写故障 - resources

%MicroCBR
% 网络故障，CPU 故障，硬盘读写故障 - resources
% 配置故障 - config

%CloudRCA
% 存储模块故障，主机硬件故障（cpu，内存）网络问题，资源调度问题（资源预占用，节点超载） - resources

%ICWS20
% 计算资源耗尽，网络延迟，网络传输中断 - resources

%LARDA
% 网络故障，CPU 故障 - resources

%LogCLuster
% 网络故障，CPU 故障 - resources

%LogCLuster
% 网络断连，磁盘满 - resources
% 机器宕机 - infrastructure dependency

%LogKG
% 内存，磁盘，网络故障，CPU 故障 - resources

%TraceRank
% 网络延迟，磁盘IO过载，CPU 资源耗尽 - resources；
